Deep Separability of Ontological Constraints

When data schemata are enriched with expressive constraints that aim at representing the domain of interest, in order to answer queries one needs to consider the logical theory consisting of both the data and the constraints. Query answering in such a context is called ontological query answering. Commonly adopted database constraints in this field are tuple-generating dependencies (TGDs) and equality-generating dependencies (EGDs). It is well known that their interaction leads to intractability or undecidability of query answering even in the case of simple subclasses. Several conditions have been found to guarantee separability, that is lack of interaction, between TGDs and EGDs. Separability makes EGDs (mostly) irrelevant for query answering and therefore often guarantees tractability, as long as the theory is satisfiable. In this paper we review the two notions of separability found in the literature, as well as several syntactic conditions that are sufficient to prove them. We then shed light on the issue of satisfiability checking, showing that under a sufficient condition called deep separability it can be done by considering the TGDs only. We show that, fortunately, in the case of TGDs and EGDs, separability implies deep separability. This result generalizes several analogous ones, proved ad hoc for particular classes of constraints. Applications include the class of sticky TGDs and EGDs, for which we provide a syntactic separability condition which extends the analogous one for linear TGDs; preliminary experiments show the feasibility of query answering in this case.

==> separability-sticky.tex <==
\section{Separability}
\label{sec:separability}
%

In this section, we exhibit a sufficient syntactic condition for
separability between sticky sets of TGDs and sets of EGDs. Before we
proceed further, let us first give the formal definition of
separability (see, e.g.,~\cite{CaGP10c}).
%
In the rest of the paper, for brevity, given a set $\dep$ of
dependencies we will denote as $\tdep$ and $\edep$ the set of TGDs
and EGDs of $\dep$, respectively.

\begin{definition}\label{def:separability}
Consider a set $\dep$ of dependencies over a schema $\R$. We say
that $\dep$ is \emph{separable} if, for every database $D$ for $\R$,
$\chase{D}{\dep}$ fails implies that $\chase{D}{\dep} \models Q$ iff
$\chase{D}{\tdep} \models Q$, for every BCQ $Q$ over $\R$. \qed
\end{definition}

We now introduce EGDs which are \emph{non-conflicting} with a sticky
set of TGDs. Before we proceed further, we need to give some
preliminary definitions. First, we recall the notion of
\emph{affected positions} of a relational schema w.r.t.~a set of
TGDs~\cite{CaGK08}.
%
Given a schema $\R$, and a set $\tdep$ of TGDs over $\R$, an
\emph{affected position} of $\R$ w.r.t.~$\tdep$ is defined
inductively as follows. Let $\pi_h$ be a position in the head of a
TGD $\sigma \in \tdep$. If an existentially quantified variable
occurs at $\pi_h$, then $\pi_h$ is affected w.r.t.~$\tdep$. If the
same universally quantified variable $X$ appears both in position
$\pi_h$, and in the body of $\sigma$ at affected positions
\emph{only}, then $\pi_h$ is affected w.r.t.~$\tdep$.
%
Intuitively speaking, the affected positions of a schema w.r.t.~a
set $\tdep$ of TGDs, are those positions at which a labeled null may
occur during the construction of the chase under $\tdep$.

A key notion is the well-known query containment under TGDs.  In
particular, given a set $\tdep$ of TGDs over a schema $\R$, and two
CQs $Q_1$ and $Q_2$ over $\R$, we say that $Q_1$ is contained in
$Q_2$ w.r.t.~$\tdep$, written $Q_1 \subseteq_{\tdep} Q_2$, if
$Q_1(D) \subseteq Q_2(D)$, for every database $D$ for $\R$ that
satisfies $\tdep$.  Notice that the problems of query containment
and of query answering (the latter in its decision version,
a.k.a.~query output tuple problem) are mutually
\textsc{logspace}-reducible~\cite{CaGK08}, and thus they have the
same complexity.

We now recall the notion of applicability of a TGD to an
atom~\cite{WCGP10}. Consider a TGD $\sigma$ over a schema $\R$, and
a set $A$ of atoms over $\R$. We say that $\sigma$ is
\emph{$A$-applicable} to an atom $\atom{a} \in A$ if the following
conditions are satisfied: \emph{(i)} $\atom{a}$ and $\head{\sigma}$
unify (recall that we consider w.l.o.g. TGDs with just one atom in
the head), \emph{(ii)} if the term at position $\pi$ in $\atom{a}$
is either a constant of $\dom$, or a variable that occurs in some
atom of $A$ other than $\atom{a}$, then the variable at position
$\pi$ in $\head{\sigma}$ occurs also in $\body{\sigma}$, and
\emph{(iii)} if a variable of $A$ occurs only in $\atom{a}$ at
positions $\pi_1,\ldots,\pi_m$, for $m \geqslant 2$, then either the
variable at position $\pi_i$ in $\head{\sigma}$, for each $i \in
[m]$, occurs also in $\body{\sigma}$, or at positions
$\pi_1,\ldots,\pi_m$ in $\head{\sigma}$ we have the same
existentially quantified variable.

Consider now a set $A$ of atoms over a schema $\R$, a variable $X$
which occurs in $A$, called the \emph{watched variable} of $A$, and
a sticky set $\tdep$ of TGDs over $\R$. By applying a procedure,
called $\mathsf{Expansion}$, which is actually a modified version of
the rewriting algorithm given in~\cite{WCGP10}, we construct the
\emph{expanded set} of $A$ w.r.t. $\tdep$. Formally,
$\mathsf{Expansion}(A,X,\tdep)$ consists of the following steps:
\begin{enumerate}\itemsep-\parsep
\item Let $S = \{\tup{A,\mathsf{id}}\}$, where $\mathsf{id}$ is the identity substitution on the terms of $A$.
%
\item Let $S' = S$.
%
\item For each pair $\tup{A,\lambda} \in S'$ apply the
following two steps:
\begin{itemize}
\item[(a)] For each $\atom{a},\atom{b} \in A$: if $\atom{a}$ and
$\atom{b}$ unify, then add to $S$ the pair $\tup{\gamma(A),\gamma
\circ \lambda}$, where $\gamma = \mathit{MGU}(\atom{a},\atom{b})$,
only if there is no $\tup{A',\lambda'} \in S$, and a bijective
(renaming) substitution $\rho$ that maps $\gamma(\lambda(X))$ to
$\lambda'(X)$, such that $\rho(\gamma(A)) = A'$.
%
\item[(b)] For each pair $\tup{\atom{a},\sigma} \in A \times \tdep$:
if \emph{(i)} $\sigma$ is $A$-applicable to $\atom{a}$; in the
sequel let $\gamma = \mathit{MGU}(\atom{a},\head{\sigma})$,
\emph{(ii)} $\widehat{A}$ contains the variable
$\gamma(\lambda(X))$, where $\widehat{A} = \gamma(A')$ and $A'$ is
obtained from $A$ by replacing the atom $\atom{a}$ with
$\body{\sigma}$, and \emph{(iii)} all the occurrences of
$\gamma(\lambda(X))$ in $\widehat{A}$ appear at affected positions
of $\R$ w.r.t. $\tdep$, then add to $S$ the pair
$\tup{\widehat{A},\gamma \circ \lambda}$, only if there is no
$\tup{A',\lambda'} \in S'$, and a bijective (renaming) substitution
$\rho$ that maps $\gamma(\lambda(X))$ to $\lambda'(X)$, such that
$\rho(\widehat{A}) = A'$.
\end{itemize}
%
\item If $S = S'$, then return $S$; otherwise, goto 2.
\end{enumerate}

Notice that at step 3b we assume w.l.o.g. that the TGD $\sigma$ and
the set $S'$ have no variables in common; we can simply rename (or
\emph{standardize apart}, in Logic Programming parlance) the
variables of $\sigma$.  This is needed to avoid clutter among
variable names introduced during different applications of step 3b.
%
Let us clarify that steps~3a and~3b correspond to \emph{minimization}
and \emph{rewriting} steps, respectively, of the rewriting algorithm
presented in~\cite{WCGP10}.
%
We now formally define non-conflicting sets of sticky TGDs and EGDs.

\begin{definition}\label{def:non-conflicting}
Consider a set $\dep$ of sticky TGDs and EGDs over a schema $\R$.
$\dep$ is \emph{non-conflicting} if, for each $\eta \in \edep$ of
the form $\varphi(\insX) \ra X_i = X_j$, the following condition
holds: for each pair $\tup{A,\lambda} \in
\mathsf{Expansion}(\mu(\varphi(\insX)),X_i,\tdep)$, for $\mu = \{X_j
\ra X_i\}$, it holds that $Q_1 \subseteq_{\tdep} Q_2$, where $Q_1$
and $Q_2$ are the conjunctive queries $q(\insY) \la
\lambda(\varphi(\insX))$ and $q(\insY) \la A$, respectively, where
$\insY$ are the variables that appear both in
$\lambda(\varphi(\insX))$ and $A$. \qed
\end{definition}

\begin{example}\label{exa:non-conflicting}
Consider the set $\dep$ consisting by
\[
\begin{array}{rcl}
\sigma_1 &:& s(X_1,Y_1)  \ra  r(Y_1,X_1),\\
%
\sigma_2 &:& p(X_2)  \ra  \exists Y_2 \, s(Y_2,X_2),\\
%
\sigma_3 &:& t(X_3,Y_3)  \ra  r(X_3,Y_3),\\
%
\sigma_4 &:& r(X_4,Y_4)  \ra  s(Y_4,X_4),\\
%
\eta &:& r(X_5,Y_5),r(X_5,Z_5) \ra Y_5=Z_5.
\end{array}
\]
The expanded set $S$ of $\mu(\body{\eta})$, where $\mu = \{Z_5 \ra
Y_5\}$, consists of the pairs
\[
\tup{\{r(X_5,Y_5)\},\mathsf{id}} \quad \textrm{~and~} \quad
\tup{\{s(Y_5,X_5)\},\{Y_1 \ra X_5, X_1 \ra Y_5\}}.
\]
%
Notice that $\tup{\{t(X_5,Y_5)\},\{X_3 \ra X_5, Y_3 \ra Y_5\}}$ is
not added to $S$ since the watched variable $Y_5$ occurs in
$t(X_5,Y_5)$ at a non-affected position, while the pair
$\tup{\{p(X_5)\},\{Y_2 \ra Y_5,X_2 \ra X_5, Y_1 \ra X_5, X_1 \ra
Y_5\}}$ is not added since $p(X_5)$ does not contain the watched
variable $Y_5$.
%
It is not difficult to verify that $Q_1 \subseteq_{\tdep} Q_2$ and
$Q_1 \subseteq_{\tdep} Q_3$, where
\[
\begin{array}{rcl}
Q_1 &:& q(X_5,Y_5) \la r(X_5,Y_5),r(X_5,Z_5),\\
%
Q_2 &:& q(X_5,Y_5) \la r(X_5,Y_5),\\
%
Q_3 &:& q(X_5,Y_5) \la s(Y_5,X_5).
\end{array}
\]
Consequently, $\dep$ is non-conflicting. \hfill\markfull
\end{example}

%\paragraph{Identifying Non-Conflicting Sets.}
Recall that $\mathsf{Expansion}$ is a modified version of the
rewriting algorithm given in~\cite{WCGP10}. Since this algorithm
terminates under sticky sets of TGDs~\cite{WCGP10} we get that the
expanded set of the body-atoms of an EGD w.r.t.~a sticky set of TGDs
is always finite. Moreover, since conjunctive query containment
under sticky sets of TGDs is decidable~\cite{CaGP10a}, we get that
the problem of identifying non-conflicting sets of sticky TGDs and
EGDs is decidable.

%\paragraph{Non-Conflicting Sets are Separable.}
Let us now establish that non-conflicting sets of sticky TGDs and
EGDs are indeed separable. Before we proceed further, let us
establish an auxiliary technical lemma.

\begin{lemma}\label{lem:auxiliary-lemma-1}
Consider a non-conflicting set $\dep$ of sticky TGDs and EGDs over
$\R$. If $\chase{D}{\dep}$ does not fail, then there exists a
homomorphism that maps $\chase{D}{\dep}$ into $\chase{D}{\tdep}$,
for every database $D$ for $\R$.
\end{lemma}

\begin{proofsketch}
The proof is by induction on the number of applications of the (TGD
or EGD) chase rule. We can show that, for each $k \geqslant 0$,
there exists a homomorphism $h_k$ such that
$h_k(\apchase{k}{D}{\dep}) \subseteq \chase{D}{\tdep}$, where
$\apchase{k}{D}{\dep}$ is the part of the chase obtained by applying
$k$ times either the TGD or the EGD chase rule. \qed
\end{proofsketch}

Our main result follows by exploiting the above technical lemma.

\begin{theorem} \label{the:separability}
Consider a set $\dep$ of sticky TGDs and EGDs over a schema $\R$. If
$\dep$ is non-conflicting, then it is also separable.
\end{theorem}

\begin{proof}
Let $D$ be a database for $\R$ such that $\chase{D}{\dep}$ does not
fail. Clearly, by construction, $\chase{D}{\dep}$ satisfies all the
dependencies in $\dep$. Therefore, $\chase{D}{\dep} \in
\mods{D}{\dep} \subseteq \mods{D}{\tdep}$. Since $\chase{D}{\tdep}$
is a universal model of $D$ w.r.t.~$\tdep$ we immediately get that
there exists a homomorphism $h$ such that $h(\chase{D}{\tdep})
\subseteq \chase{D}{\dep}$.
%
On the other hand, Lemma~\ref{lem:auxiliary-lemma-1} implies that
there exists a homomorphism $h'$ such that $h'(\chase{D}{\dep})
\subseteq \chase{D}{\tdep}$.
%
Due to the existence of $h$ and $h'$ it holds that, for every BCQ
$Q$ over $\R$, $\chase{D}{\dep} \models Q$ iff $\chase{D}{\tdep}
\models Q$. \qed
\end{proof}

%\paragraph{Query Answering under Non-Conflicting Sets.}
We conclude this subsection by investigating the \emph{data} and
\emph{combined complexity} of BCQ answering under non-conflicting
sets of sticky TGDs and EGDs. Recall that the data complexity is
calculated by considering only the data as input, while the combined
complexity is calculated by considering also the query and the
dependencies as part of the input.

\begin{theorem}\label{the:bcq-answering-under-non-conflicting-sets}
Consider a BCQ $Q$ over a schema $\R$, a database $D$ for $\R$, and
a non-conflicting set $\dep$ of sticky TGDs and EGDs over $\R$. The
problem whether $D \cup \dep \models Q$ is in \textsc{ac}$^0$ in
data complexity, and is \textsc{exptime}-complete in combined
complexity.
\end{theorem}

\begin{proofsketch}
Suppose that $\chase{D}{\dep}$ does not fail. By
Theorem~\ref{the:separability}, we get that $D \cup \dep \models Q$,
or, equivalently, $\chase{D}{\dep} \models Q$ iff $\chase{D}{\tdep}
\models Q$. It is well-known that BCQ answering under sticky TGDs is
in \textsc{ac}$^0$ in data complexity, and \textsc{exptime}-complete
in combined complexity~\cite{CaGP10a}. Since $\tdep$ is a set of
sticky TGDs, providing that the chase does not fail, the desired
complexity follows.
%
Since the problem whether $\chase{D}{\dep}$ fails is tantamount to
BCQ answering under sticky TGDs (see, e.g.,~\cite{CaGP10c}), the
claim follows. \qed
\end{proofsketch}

As shown in~\cite{CaGP10a}, it is possible to combine sticky TGDs
with \emph{negative constraints} of the form $\forall \insX
\varphi(\insX) \ra \bot$, without altering the computational
complexity of BCQ answering. By exploiting this result, we can also
show that non-conflicting sets of sticky TGDs and EGDs can be
combined with negative constraints, without paying a price in
complexity of query answering.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

